Leveraging phone-level linguistic-acoustic similarity for utterance-level pronunciation scoring

Recent studies on pronunciation scoring have explored the effect of introducing phone embeddings as reference pronunciation, but mostly in an implicit manner, i.e., addition or concatenation of reference phone embedding and actual pronunciation of the target phone as the phone-level pronunciation quality representation. In this paper, we propose to use linguistic-acoustic similarity to explicitly measure the deviation of non-native production from its native reference for pronunciation assessment. Specifically, the deviation is first estimated by the cosine similarity between reference phone embedding and corresponding acoustic embedding. Next, a phone-level Goodness of pronunciation (GOP) pre-training stage is introduced to guide this similarity-based learning for better initialization of the aforementioned two embeddings. Finally, a transformer-based hierarchical pronunciation scorer is used to map a sequence of phone embeddings, acoustic embeddings along with their similarity measures to predict the final utterance-level score. Experimental results on the non-native databases suggest that the proposed system significantly outperforms the baselines, where the acoustic and phone embeddings are simply added or concatenated. A further examination shows that the phone embeddings learned in the proposed approach are able to capture linguistic-acoustic attributes of native pronunciation as reference.

==> content/sections/misc.tex <==
\begin{table}[h]
\centering
\resizebox{0.7\columnwidth}{!}{
\begin{tabular}{c|cc}
\toprule
                                          & \multicolumn{2}{c}{Datasets}      \\ \cline{2-3} 
\multirow{-2}{*}{Methods}                 & ez10k           & speechocean762     \\ \midrule
add\_phone                                & 0.7637          & 0.5979          \\
concat\_phone                             & 0.7629          & 0.6180          \\ \hline
\textbf{Proposed} & \textbf{0.8252} & \textbf{0.6437} \\
\bottomrule
\end{tabular}
}
\caption{The PCC results of the proposed method compared with that of \textit{add\_phone} and \textit{concat\_phone} on two datasets.}
\end{table}

